On the Estimation and Control of Human Body Composition

Obesity is a chronic disease that can lead to an increased risk of other serious chronic diseases and even death. We present switching and time-delayed feedback-based model free control methods for the dynamic management of body mass and its major components. The estimation of body composition based on human body weight dynamics is proposed using a soft switching-based observer. Additionally, this paper addresses the control allocation problem for optimal body weight management using linear algebraic equivalence of the nonlinear controllers based on dynamic behavior of body composition described in literature. A control allocator system computes the required energy intake and energy expenditure from a controlling range of inputs to track a desired trajectory of body mass by optimizing a weighted quadratic function. Simulation results validate the performance of the proposed controllers and the observer under disturbances in recording energy intake and energy expenditure figures.

==> defns.tex <==
%% 
%% Common definitions
%% Only contains the definitions, not formatting information
%%

\usepackage{xspace}
\usepackage{bbm}
%\usepackage{mathrsfs}
%% \usepackage{semantic}
%% \usepackage{bm}
\input{mathlig}

%% Small spacing
\newcommand{\muspace}{\mspace{1mu}}

%% |
\DeclareRobustCommand{\scond}{\mathchoice{\muspace\vert\muspace}{\vert}{\vert}{\vert}}
\mathlig{|}{\scond}
\newcommand{\cond}{\mathchoice{\,\vert\,}{\mspace{2mu}\vert\mspace{2mu}}{\vert}{\vert}}
\newcommand{\bigcond}{\,\big\vert\,}

%% :
\DeclareRobustCommand{\discint}{\mathchoice{\mspace{-1.5mu}:\mspace{-1.5mu}}{\mspace{-1.5mu}:\mspace{-1.5mu}}{:}{:}}
\mathlig{::}{\discint}
\newcommand{\suchthat}{\mathchoice{\colon}{\colon}{:\mspace{1mu}}{:}}
\newcommand{\mappingfrom}{\colon}

%% A few operator definitions
\def\tr{\mathop{\rm tr}\nolimits}%
\def\var{\mathop{\rm Var}\nolimits}%
\def\Var{\mathop{\rm Var}\nolimits}%
\def\cov{\mathop{\rm Cov}\nolimits}%
\def\Cov{\mathop{\rm Cov}\nolimits}%
\def\diag{\mathop{\rm diag}\nolimits}%
\def\Re{\mathop{\rm Re}\nolimits}%
\def\Im{\mathop{\rm Im}\nolimits}%
\def\rank{\mathop{\rm rank}\nolimits}%
\def\essinf{\mathop{\rm ess\,inf}}%
\def\sgn{\mathop{\rm sgn}\nolimits}%
\def\erfc{\mathop{\rm erfc}\nolimits}%
\def\co{\mathop{\rm co}\nolimits}%

%% Mathcal (discrete sets)
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\cc}{\text{\footnotesize $\mathcal{C}$} }
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mspace{1.5mu}\mathcal{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

%% Mathcal bold (random discrete sets)
\newcommand{\Acb}{\boldsymbol{\mathcal{A}}}
\newcommand{\Bcb}{\boldsymbol{\mathcal{B}}}
\newcommand{\Ccb}{\boldsymbol{\mathcal{C}}}
\newcommand{\Dcb}{\boldsymbol{\mathcal{D}}}
\newcommand{\Ecb}{\boldsymbol{\mathcal{E}}}
\newcommand{\Fcb}{\boldsymbol{\mathcal{F}}}
\newcommand{\Gcb}{\boldsymbol{\mathcal{G}}}
\newcommand{\Hcb}{\boldsymbol{\mathcal{H}}}
\newcommand{\Jcb}{\boldsymbol{\mathcal{J}}}
\newcommand{\Kcb}{\boldsymbol{\mathcal{K}}}
\newcommand{\Ncb}{\boldsymbol{\mathcal{N}}}
\newcommand{\Pcb}{\boldsymbol{\mathcal{P}}}
\newcommand{\Qcb}{\boldsymbol{\mathcal{Q}}}
\newcommand{\Rcb}{\boldsymbol{\mathcal{R}}}
\newcommand{\Scb}{\boldsymbol{\mathcal{S}}}
\newcommand{\Tcb}{\boldsymbol{\mathcal{T}}}
\newcommand{\Ucb}{\boldsymbol{\mathcal{U}}}
\newcommand{\Vcb}{\boldsymbol{\mathcal{V}}}
\newcommand{\Wcb}{\boldsymbol{\mathcal{W}}}
\newcommand{\Xcb}{\boldsymbol{\mathcal{X}}}
\newcommand{\Ycb}{\boldsymbol{\mathcal{Y}}}
\newcommand{\Zcb}{\boldsymbol{\mathcal{Z}}}


%% Script sets: Capacity region, set of probs, achievable rate region, etc.
\newcommand{\Ar}{\mathscr{A}}
\newcommand{\Cr}{\mathscr{C}}
\newcommand{\Dr}{\mathscr{D}}
\renewcommand{\Pr}{\mathscr{P}}
\newcommand{\Rr}{\mathscr{R}}
\newcommand{\Ur}{\mathscr{U}}
\newcommand{\Kr}{\mathscr{K}}
\newcommand{\Gr}{\mathscr{G}}
\newcommand{\Sr}{\mathscr{S}}
%% Sequences
%% TODO: Should be cleaned up
\iffalse
\newcommand{\Un}{{U_1,U_2,\ldots,U_n}}
\newcommand{\Vn}{{V_1,V_2,\ldots,V_n}}
\newcommand{\Xk}{{X^{(1)},X^{(2)},\ldots,X^{(k)}}}
\newcommand{\xk}{{x^{(1)},x^{(2)},\ldots,x^{(k)}}}
\newcommand{\Xm}{{X^{(1)},X^{(2)},\ldots,X^{(m)}}}
\newcommand{\xm}{{x^{(1)},x^{(2)},\ldots,x^{(m)}}}
\newcommand{\Xn}{{X_1,X_2,\ldots,X_n}}
\newcommand{\xn}{{x_1,x_2,\ldots,x_n}}
\newcommand{\Ym}{{Y^{(1)},Y^{(2)},\ldots,Y^{(m)}}}
\newcommand{\ym}{{y^{(1)},y^{(2)},\ldots,y^{(m)}}}
\newcommand{\Yn}{{Y_1,Y_2,\ldots,Y_n}}
\newcommand{\yn}{{y_1,y_2,\ldots,y_n}}
\newcommand{\Zn}{{Z_1,Z_2,\ldots,Z_n}}
\newcommand{\zn}{{z_1,z_2,\ldots,z_n}}
\fi


%% Boldface vectors
%%
\newcommand{\Lv}{{\bf L}}
\newcommand{\Xv}{{\bf X}}
\newcommand{\Yv}{{\bf Y}}
\newcommand{\Zv}{{\bf Z}}
\newcommand{\Uv}{{\bf U}}
\newcommand{\Wv}{{\bf W}}
\newcommand{\Vv}{{\bf V}}
\newcommand{\Sv}{{\bf S}}
\newcommand{\av}{{\bf a}}
\newcommand{\bv}{{\bf b}}
\newcommand{\cv}{{\bf c}}
\newcommand{\fv}{{\bf f}}
\newcommand{\gv}{{\bf g}}
\newcommand{\lv}{{\boldsymbol l}}
\newcommand{\mv}{{\bf m}}
\newcommand{\xv}{{\bf x}}
\newcommand{\yv}{{\bf y}}
\newcommand{\zv}{{\bf z}}
\newcommand{\uv}{{\bf u}}
\newcommand{\vv}{{\bf v}}
\newcommand{\sv}{{\bf s}}
\newcommand{\alphav}{{\boldsymbol \alpha}}
\newcommand{\betav}{{\boldsymbol \beta}}
\newcommand{\gammav}{{\boldsymbol \gamma}}
\newcommand{\lambdav}{{\boldsymbol \lambda}}
\newcommand{\muv}{{\boldsymbol \mu}}
\newcommand{\nuv}{{\boldsymbol \nu}}
\newcommand{\onev}{{\boldsymbol 1}}


%% Typicality
%% \newcommand{\feq}{\stackrel{.}{=}}
\newcommand{\pen}{{P_e^{(n)}}}
\newcommand{\waep}{{\mathcal{A}_{\epsilon}^{(n)}}}
\newcommand{\aep}{{\mathcal{T}_{\epsilon}^{(n)}}}
\newcommand{\aepvar}{{\mathcal{T}_{\epsilon'}^{(n)}}}
\newcommand{\aepvarvar}{{\mathcal{T}_{\epsilon''}^{(n)}}}
\newcommand{\aepk}{{\mathcal{T}_{\epsilon}^{(k)}}}
\newcommand{\aepd}{{\mathcal{T}_{\delta(\epsilon)}^{(n)}}}

%% Hats
\newcommand{\Kh}{{\hat{K}}}
\newcommand{\Lh}{{\hat{L}}}
\newcommand{\Mh}{{\hat{M}}}
\newcommand{\Rh}{{\hat{R}}}
\newcommand{\Sh}{{\hat{S}}}
\newcommand{\Uh}{{\hat{U}}}
\newcommand{\Vh}{{\hat{V}}}
\newcommand{\Wh}{{\hat{W}}}
\newcommand{\Xh}{{\hat{X}}}
\newcommand{\Yh}{{\hat{Y}}}
\newcommand{\Zh}{{\hat{Z}}}
\renewcommand{\dh}{{\hat{d}}}
\newcommand{\kh}{{\hat{k}}}
\newcommand{\lh}{{\hat{l}}}
\newcommand{\mh}{{\hat{m}}}
\newcommand{\sh}{{\hat{s}}}
\newcommand{\uh}{{\hat{u}}}
\newcommand{\vh}{{\hat{v}}}
\newcommand{\wh}{{\hat{w}}}
\newcommand{\xh}{{\hat{x}}}
\newcommand{\yh}{{\hat{y}}}
\newcommand{\zh}{{\hat{z}}}
\newcommand{\gh}{{\hat{g}}}
%% Tildes
\newcommand{\At}{{\tilde{A}}}
\newcommand{\Ct}{{\tilde{C}}}
\newcommand{\Kt}{{\tilde{K}}}
\newcommand{\Lt}{{\tilde{L}}}
\newcommand{\Mt}{{\tilde{M}}}
\newcommand{\Nt}{{\tilde{N}}}
\newcommand{\Qt}{{\tilde{Q}}}
\newcommand{\Rt}{{\tilde{R}}}
\newcommand{\St}{{\tilde{S}}}
\newcommand{\Ut}{{\tilde{U}}}
\newcommand{\Vt}{{\tilde{V}}}
\newcommand{\Wt}{{\tilde{W}}}
\newcommand{\Xt}{{\tilde{X}}}
\newcommand{\Yt}{{\tilde{Y}}}
\newcommand{\Zt}{{\tilde{Z}}}
\newcommand{\dt}{{\tilde{d}}}
\newcommand{\kt}{{\tilde{k}}}
\newcommand{\lt}{{\tilde{l}}}
\newcommand{\mt}{{\tilde{m}}}
\newcommand{\pt}{{\tilde{p}}}
\newcommand{\rt}{{\tilde{r}}}
\newcommand{\st}{{\tilde{s}}}
\newcommand{\ut}{{\tilde{u}}}
\newcommand{\vt}{{\tilde{v}}}
\newcommand{\wt}{{\tilde{w}}}
\newcommand{\xt}{{\tilde{x}}}
\newcommand{\yt}{{\tilde{y}}}
\newcommand{\zt}{{\tilde{z}}}
\newcommand{\gt}{{\tilde{g}}}

%% Greek
\def\a{\alpha}
\def\b{\beta}
\def\g{\gamma}
\def\d{\delta}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\l{\lambda}
\def\th{\theta}
\def\Th{\Theta}

%% Probability and expectation
\DeclareMathOperator\E{\textsf{E}}
\let\P\relax
\DeclareMathOperator\P{\textsf{P}}

%% Gaussian capacity, rate-dist, binary entropy
\DeclareMathOperator\C{\textsf{C}}
\DeclareMathOperator\R{\textsf{R}}
%\DeclareMathOperator\C{C}
%\DeclareMathOperator\R{R}

%% Error symbol
\def\error{\mathrm{e}}

%% Probability distributions
%%\newcommand{\Br}{\mathrm{Bern}}
\newcommand{\Bern}{\mathrm{Bern}}
\newcommand{\Geom}{\mathrm{Geom}}
\newcommand{\Poisson}{\mathrm{Poisson}}
\newcommand{\Exp}{\mathrm{Exp}}
%%\newcommand{\Norm}{\mathrm{N}}
\newcommand{\N}{\mathrm{N}}
\newcommand{\U}{\mathrm{Unif}}
\newcommand{\B}{\mathrm{Binom}}
%% Misc
\newcommand\eg{e.g.,\xspace}
\newcommand\ie{i.e.,\xspace}
\def\textiid{i.i.d.\@\xspace}
\newcommand\iid{\ifmmode\text{ i.i.d. } \else \textiid \fi}
\let\textand\and
%\renewcommand\and{\ifmmode{\text{ and }}{\textand}}
\let\textor\or
%\renewcommand\or{\ifmmode{\text{ or }}{\textor}}
\newcommand{\geql}{\succeq}
\newcommand{\leql}{\preceq}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Ff}{\mathbb{F}}
\newcommand{\Zz}{\mathbb{Z}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\ind}{\boldsymbol{1}}
\newcommand{\defeq}{=}
\newcommand{\carddot}{\mathchoice{\!\cdot\!}{\!\cdot\!}{\cdot}{\cdot}}

%%------------------------------------------------------- 
%% Fractions
%%
\newcommand{\sfrac}[2]{\mbox{\small$\displaystyle\frac{#1}{#2}$}}
\newcommand{\half}{\sfrac{1}{2}}

%%------------------------------------------------------- 
%% Cups and caps
%%
\def\medcupmath{\mbox{\small$\displaystyle\bigcup$}}
\def\medcuptext{\raisebox{1pt}{\small$\textstyle\bigcup$}}
\def\medcup{\mathop{\mathchoice{\medcupmath}{\medcuptext}{\bigcup}{\bigcup}}}

\def\medcapmath{\raisebox{0.5pt}{\small$\displaystyle\bigcap$}}
\def\medcaptext{\raisebox{1pt}{\small$\textstyle\bigcap$}}
\def\medcap{\mathop{\mathchoice{\medcapmath}{\medcaptext}{\bigcap}{\bigcap}}}


%%------------------------------------------------------- 
%% Products
%%
\def\medtimesmath{\mbox{\small$\displaystyle\bigtimes$}}
\def\medtimestext{\raisebox{1pt}{\small$\textstyle\bigtimes$}}
\def\medtimes{\mathop{\mathchoice{\medtimesmath}{\medtimestext}{\bigtimes}{\bigtimes}}}


%%--------------------------------------------------------
%% Spacing
%%
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathllapinternal#1#2{%
  \llap{$\mathsurround=0pt#1{#2}$}}

\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathrlapinternal#1#2{%
  \rlap{$\mathsurround=0pt#1{#2}$}}

\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathclapinternal#1#2{%
  \clap{$\mathsurround=0pt#1{#2}$}}

%% For lecture notes
\def\labelitemi{$\bullet$}
\def\labelitemii{$\bullet$}
%\def\labelitemii{$\circ$}

%%-------------------------------------------------------
%% Stackrel
%%

\let\oldstackrel\stackrel
\renewcommand{\stackrel}[2]{\oldstackrel{\mathclap{#1}}{#2}}

%-------------------------------------------------------------------------
% Interchapter macros

\newcommand{\Csum}{C_\mathrm{sum}}
\newcommand{\Csym}{C_\mathrm{sym}}
\newcommand{\Ccc}{C_\mathrm{CC}}
\newcommand{\Cavc}{C_\mathrm{AVC}}
\newcommand{\Cnsi}{C_\mathrm{NSI}}
\newcommand{\CXX}[3]{{#1}_{\mathrm{#2\text{-}#3}}}
\newcommand{\Csid}{\CXX{C}{SI}{D}}
\newcommand{\Csie}{\CXX{C}{SI}{E}}
\newcommand{\Csied}{\CXX{C}{SI}{ED}}
\newcommand{\Ccsie}{\CXX{C}{CSI}{E}}
\newcommand{\Crsid}{\CXX{\Cr}{SI}{D}}
\newcommand{\Crsied}{\CXX{\Cr}{SI}{ED}}
\newcommand{\Crdsied}{\CXX{\Cr}{DSI}{ED}}

\newcommand{\Rsid}{\CXX{R}{SI}{D}}
\newcommand{\Rcsid}{\CXX{R}{CSI}{D}}
\newcommand{\Rcsied}{\CXX{R}{CSI}{ED}}
\newcommand{\Rsied}{\CXX{R}{SI}{ED}}
\newcommand{\Rsie}{\CXX{R}{SI}{E}}

\newcommand{\Rs}{R_\mathrm{s}}
\newcommand{\Ms}{M_\mathrm{s}}
\newcommand{\ms}{m_\mathrm{s}}
\newcommand{\mk}{m_\mathrm{K}}

\newcommand{\Rcfo}{R_\mathrm{CFO}}
\newcommand{\Rrcfo}{\Rr_\mathrm{CFO}}
\newcommand{\Cs}{C_\mathrm{S}}
\newcommand{\Ck}{C_\mathrm{K}}
\newcommand{\Rk}{R_\mathrm{K}}
\newcommand{\Rl}{R_\mathrm{L}}
\newcommand{\Rln}{R_\mathrm{L}^{(n)}}
\newcommand{\Ckone}{C_\mathrm{K}^{(1)}}
\newcommand{\Ckq}{C_\mathrm{K}^{(q)}}
\newcommand{\Ckow}{\CXX{C}{K}{OW}}
\newcommand{\Ckcm}{\CXX{C}{K}{CM}}

\newcommand{\musum}{$\muv$\nobreakdash-sum}
%-------------------------------------------------------------------------
% PSFrag vertical adjustment

\newcommand{\adjas}[2]{\smash{#1}\vphantom{#2}}
\newcommand{\adjasm}[1]{\adjas{#1}{$m$}}
\newcommand{\adjasM}[1]{\adjas{#1}{$M$}}

%-------------------------------------------------------------------------
% Overline
\newcommand{\Hbar}{H\mathllap{\overline{\vphantom{H}\hphantom{\rule{6.9pt}{0pt}}}\mspace{0.7mu}}}
\newcommand{\Gbar}{G\mathllap{\overline{\vphantom{G}\hphantom{\rule{6.25pt}{0pt}}}\mspace{1.1mu}}}
\renewcommand{\hbar}{h\mathllap{\overline{\vphantom{h}\hphantom{\rule{4.6pt}{0pt}}}\mspace{0.77mu}}}

%------------------------------------
% URL tilde
\catcode`~=11 % make LaTeX treat tilde (~) like a normal character
\newcommand{\urltilde}{\kern -.06em\lower -.06em\hbox{~}\kern .02em}
\catcode`~=13 % revert back to treating tilde (~) as an active character


%------------------------------------
% Hyphenation
\hyphenation{Gauss-ian}
\hyphenation{qua-dra-tic}
\hyphenation{Vis-wa-nath}
\hyphenation{non-trivial}
\hyphenation{multi-letter}
\hyphenation{Gauss-ian}
\hyphenation{super-posi-tion}
\hyphenation{de-cod-er}
\hyphenation{Nara-yan}
\hyphenation{multi-message}
\hyphenation{Dimi-tris}
\hyphenation{Pol-ty-rev}
\hyphenation{multi-cast}
\hyphenation{multi-user}
\hyphenation{multi-plex-ing}
\hyphenation{bi-directional}
\hyphenation{comput}

==> harvard/README <==
# harvard family of bibliographic styles
# Copyright 1994 - Peter Williams pwil3058@bigpond.net.au
#
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
# 
# The Current Maintainers of this work are Peter Williams and Thorsten Schnier.
#
# This work consists of all files listed in manifest.txt.
#
# Licence notice added on behalf of Peter Williams and Thorsten Schnier
# by Clea F. Rees 2009/01/30.

This is version 2.0.5 of the harvard family of bibliographic styles.
It is a bug fix of 2.0 which was a major rewrite to bring the sty file into
line with the new latex described in ``The LaTeX Companion''.  Due to the
efforts of Thorsten Schnier (thorsten@archsci.arch.su.edu.au) it incorporates
support for the LaTeX to html translator by Nikos Drakos
(nikos@cbl.leeds.ac.uk).

It includes a fixes by Berwin A. Turlach (berwin@alphasun.anu.edu.au) for
problems with \AtBeginDocument introduced in the latest version of LaTeX2e
and problems with the \nocite command.

A new style apsr.bst (American Political Science Review) is enclosed
courtesy of Nathaneil L. Beck (nbeck@weber.ucsd.edu)

NB.  The file harvard.sty makes considerable use of features in the new latex
that were not present in latex version 2.09 and is, therefore, not compatible
with that version.  However, the *.bbl files produced by the various bst files
should be still useable with latex version 2.09.

The following files are enclosed.

  README	- This file
  INSTALL	- Installation instructions
  Makefile	- Makefile for installation
  harvard.ps	- Postscript version of the documentation
  harvard.tex	- LaTeX source for the documentation
  harvard.bib	- BibTeX database file for the documentation
  doc_Makefile	- Makefile for documentation
  harvard.sty	- LaTeX style file for harvard bibliographic style
  harvard.perl	- LaTeX2html style file for harvard bibliographic style
  agsm.bst	- harvard BibTeX style file to satisfy the requirements
		  of the Australian Government Style Manual
  dcu.bst	- harvard BibTeX style file to satisfy the requirements
		  of the Design Computing Unit, Sydney University
  <other>.bst	- various style files contributed by users

Online documentation is available via the WWW at:

HREF="http://www.arch.su.edu.au/~peterw/latex/harvard/"


==> mathlig.tex <==
%
% mathlig.tex
%
% (c) 2001 Jules Bean <jules@jellybean.co.uk>
% Permission is granted to freely use, copy, and distribute
% without restriction. Permission is also granted to distribute
% modified versions and incorporate into your own macro packages
% if a brief acknowledgement is given.
%
% Version 1.0  11 May 2001

% Define 'mathmode' ligatures, as in 
%
%\mathlig{->}{\rightarrow}
%\mathlig{<-}{\leftarrow}
%\mathlig{<->}{\leftrightarrow}
%
% Works even if they have common prefixes (takes the longest match,
% then backtracks).
%
% Can be used to create ligatures even if the second
% and subsequent characters have weird catcodes, but I don't recommend 
% it.

\count255\catcode`@
\catcode`@=11
\chardef\mathlig@atcode\count255

% Let or def an 'active' version of a token.  Thanks to Donald
% Arseneau and groups.google.com
\def\actively#1#2{\begingroup\uccode`\~=`#2\relax\uppercase{\endgroup#1~}}
% Eat the next token, and then pass control to mathlig@next@cmd
\def\mathlig@gobble{\afterassignment\mathlig@next@cmd\let\mathlig@next= }
% Used to delimit delimited arguments, and ifx tests for emptyness.
\def\mathlig@delim{\mathlig@delim}
% Some macros to help dealing with 'computed names' (csnames).
% Just like def, but first parameter is evaluated as a csname
\def\mathlig@defcs#1{\expandafter\def\csname#1\endcsname}
% A version of \let <normal cs><computed cs>
\def\mathlig@let@cs#1#2{\expandafter\let\expandafter#1\csname#2\endcsname}
% Maintain a 'list' of tokens as a macro which expands to them
\def\mathlig@appendcs#1#2{\expandafter\edef\csname#1\endcsname{\csname#1\endcsname#2}}

% The main externally visible macro. 
% Defines '#1' as a 'ligature' to expand to #2
% First uses \mathlig@checklig to make sure that all initial segments of
% #1 as set up as ligatures.
% Then sets the ligature #1 to expand to #2.
\def\mathlig#1#2{\mathlig@checklig#1\mathlig@end\mathlig@defcs{mathlig@back@#1}{#2}\ignorespaces}

% All the @check macros should be idempotent: they set up the definitions
% only if it hasn't already been done.

%Check #1#2 can be a ligature:
% Check #1 is math-active.
% If not, save the mathcode, set the macros #1
%Now check the suffix tables with \checkrest
\def\mathlig@checklig#1#2\mathlig@end{%
 \expandafter\ifx\csname mathlig@forw@#1\endcsname\relax
 \expandafter\mathchardef\csname mathlig@back@#1\endcsname=\mathcode`#1%
 \mathcode`#1"8000\actively\def#1{\csname mathlig@look@#1\endcsname}%
 \mathlig@dolig#1\mathlig@delim
\fi
\mathlig@checksuffix#1#2\mathlig@end
}

%Two-part macro.
%Check suffix tables. If #2 is empty, no suffix!
%Otherwise, we make sure #2 is a valid suffix for #1,
%then recurse for #3 on #1#2
\def\mathlig@checksuffix#1#2\mathlig@end{%
\ifx\mathlig@delim#2\mathlig@delim\relax\else\mathlig@checksuffix@{#1}#2\mathlig@end\fi
}
\def\mathlig@checksuffix@#1#2#3\mathlig@end{%
\expandafter\ifx\csname mathlig@forw@#1#2\endcsname\relax\mathlig@dosuffix{#1}{#2}\fi
\mathlig@checksuffix{#1#2}#3\mathlig@end
}

% The do macros should not be called more than once for a given ligature.

% Add #2 to the list of valid suffixes for #1
% Then make the ligature for #1#2 one which only backtracks, for now
\def\mathlig@dosuffix#1#2{%
\mathlig@appendcs{mathlig@toks@#1}{#2}%
\mathlig@dolig{#1}{#2}\mathlig@delim
}

% Setup #1#2 so that ligatures beginning #1#2 work.
% Such ligatures will look at what's coming next (in case
% of a longer ligature) and, failing that, 
% backtrack to just #1

\def\mathlig@dolig#1#2\mathlig@delim{%
%The look macro just \futurelets what's coming up and
%then passes control to forw
 \mathlig@defcs{mathlig@look@#1#2}{%
 \mathlig@let@cs\mathlig@next{mathlig@forw@#1#2}\futurelet\mathlig@next@tok\mathlig@next}%
%The forw macro uses chck to try all possible suffixes, passing control
%either to one of those, or to the back macro
 \mathlig@defcs{mathlig@forw@#1#2}{%
  \mathlig@let@cs\mathlig@next{mathlig@back@#1#2}%
  \mathlig@let@cs\checker{mathlig@chck@#1#2}%
  \mathlig@let@cs\mathligtoks{mathlig@toks@#1#2}%
  \expandafter\ifx\expandafter\mathlig@delim\mathligtoks\mathlig@delim\relax\else
  \expandafter\checker\mathligtoks\mathlig@delim\fi
  \mathlig@next
 }%
%The toks macro just stores the suffixes
 \mathlig@defcs{mathlig@toks@#1#2}{}%
%The chk macro goes through the suffixes one by one
%tail recursing until it runs out, or finds one.
 \mathlig@defcs{mathlig@chck@#1#2}##1##2\mathlig@delim{%
  %\message{Lig so far '#1#2', checking for '##1'}%
  \ifx\mathlig@next@tok##1%
   \mathlig@let@cs\mathlig@next@cmd{mathlig@look@#1#2##1}\let\mathlig@next\mathlig@gobble
  \fi 
  \ifx\mathlig@delim##2\mathlig@delim\relax\else
   \csname mathlig@chck@#1#2\endcsname##2\mathlig@delim
  \fi
 }%
%
% The back macro, defined only if this is a ligature of at least
% two characters, is a default fallback: go back to the previous char.
% (If this is a ligature of only one character, the mathcode will have 
% been saved and set as the fallback elsewhere)
 \ifx\mathlig@delim#2\mathlig@delim\else
  \mathlig@defcs{mathlig@back@#1#2}{\csname mathlig@back@#1\endcsname #2}%
 \fi
}%

\catcode`@\mathlig@atcode

